Unraveling the Interconnected Axes of Heterogeneity in Machine Learning for Democratic and Inclusive Advancements

The growing utilization of machine learning (ML) in decision-making processes raises questions about its benefits to society. In this study, we identify and analyze three axes of heterogeneity that significantly influence the trajectory of ML products. These axes are i) values, culture and regulations, ii) data composition, and iii) resource and infrastructure capacity. We demonstrate how these axes are interdependent and mutually influence one another, emphasizing the need to consider and address them jointly. Unfortunately, the current research landscape falls short in this regard, often failing to adopt a holistic approach. We examine the prevalent practices and methodologies that skew these axes in favor of a selected few, resulting in power concentration, homogenized control, and increased dependency. We discuss how this fragmented study of the three axes poses a significant challenge, leading to an impractical solution space that lacks reflection of real-world scenarios. Addressing these issues is crucial to ensure a more comprehensive understanding of the interconnected nature of society and to foster the democratic and inclusive development of ML systems that are more aligned with real-world complexities and its diverse requirements.

==> 07_Related_work_bis.tex <==




% Democratizing artificial intelligence has become an important topic for both research and industry \cite{ahmed2020framework, nguyen2021distributed, allen2019democratizing}. Some of the key advocated principles are reusability, portability, and accessibility of AI models. These properties can be achieved through designing well documented and lightweight models. 
% Accordingly, several guidelines for documenting models \cite{mitchell2019model} and datasets \cite{gebru2021datasheets} were designed and adopted by the community. 
% Additionally, various lightweight variants of models were proposed \cite{howard2017mobilenets,kusupati_fastgrnn_2018,zhang_shufflenet_2018, sudharsan_edge2train_2020,kumar-resource-efficient-nodate}, in addition to compression techniques such as pruning \cite{blalock2020state} and quantization \cite{guo2018survey}. However, accessibility and reusability do not guarantee model performance in new contexts, mainly due to data heterogeneity. For instance, it was shown that model pruning has adverse effects on model fairness against minority groups \cite{hooker2020characterising}.


% An emerging direction is building robust models under distribution shifts \cite{schumann2019transfer, chen2022fairness,an2022transferring} and scarce data in target domain \cite{sattigeri2019fairness}. Nonetheless, several of these solutions require local expertise and specialized knowledge. A typical AI development team lacks the lived experiences required to comprehensively approximate and account for the various stakeholders, especially already marginalized communities  \cite{birhane2022power}. Participatory design allows to include feedback and expertise from the communities impacted by different AI decisions \cite{martin2020participatory}. However, ML practitioners might claim participatory design when the communities are only lightly included (e.g., one-time workshops or focus groups) \cite{zytko2022participatory}.  
% Researchers have warned against these practices and considered them as "participation-washing" \cite{sloane2020participation}. An example of stakeholders that should be given more importance in the ML pipeline are annotators. They are referred to as “ghost workers” or "data janitors" in data process pipeline \cite{gray2019ghost, irani2019justice}, and their work is faced with low compensation and lack of inclusion, which negatively impacts the quality of ML systems. 
% Democratizing AI in general, and fairness in ML in particular, requires the design of more empowering and inclusive processes. 

% To include the different values and regulations to honor the diversity of the society and build trustworthy systems, many impact assessments and principles were formulated and proposed such as the Blueprint for an AI Bill of Rights  \cite{hine2022blueprint}, the Asilomar AI Principles  \cite{future2017asilomar}, the Proposal of an EU AI Act  \cite{faupel2001charter}, and the Montreal Declaration for Responsible AI  \cite{international2011declaration}. However, principles alone are not enough even in relatively well-understood industries such as bioethics and safety engineering let alone fast-evolving AI research. Often generality of these principles limits their ability to provide practical action plans  \cite{whittlestone2019role}. Nevertheless, there is value in standardization to some extent, these frameworks can act as a decent first step and provide a common language to follow more context-dependent study but there are not sufficient on their own. 

% The goal of the democratic fairness framework is to include local values and regulations and honor diversity, on top of making ML accessible, portable and sustainable. Additionally, instead of only defining principles and guidelines, we also discuss several techniques that can be a first step towards democratizing algorithmic fairness.

% In essence, participatory approaches aim to transcend individual opinions in order to engender inclusion, collective trust and ownership, thereby shifting the dynamic of users to collaborators. It also contributes to social capacity building in the society \cite{birhane2022power}. Generally a broad range of participants plays an important role in the machine learning pipeline but the reward of this participation is disproportionately distributed among different stakeholders. A well-known example is “ghost workers” or "data janitors" in data process pipeline \cite{gray2019ghost, irani2019justice}. This uneven reward distribution naturally would cause a negative impact on the quality of our systems. 
% %A typical benchmarks datasets.


% Oftentimes more than usual participation is employed where designers experience skepticism or anticipate public resistance towards a product or service or as a means for facilitating local adaption to international development schemes \cite{sloane2020participation}. When we already started to implement our models in socially consequential domains and influencing people's lives, we should at least add elements including participation to enhance the level of model reliability. 


% Some papers suggest building a collaborative causal inference development alongside different stakeholder groups including marginalized communities to center their voices and lived experiences where they are impacted by ML-based products and understand the context of products better  \cite{martin2020participatory}. While this is truly a valuable step, it fails to account for existing power dynamics between the developing entity or "owners" and the communities. Given the extractive nature of feedback loops and the free labor put into them, this proposal calls for defined equitable reciprocity schemes and safety guarantees. Participation without redistribution of power is an empty process for the powerless. It allows the powerholders to claim inclusion, while makes it possible for few to benefit. It maintains the usual status quo to serve the powerful even more \cite{birhane2022power}. 



% Many impact assessments and principles were formulated and proposed such as the Blueprint for an AI Bill of Rights  \cite{hine2022blueprint}, the Asilomar AI Principles  \cite{future2017asilomar}, the Proposal of an EU AI Act  \cite{faupel2001charter}, and the Montreal Declaration for Responsible AI  \cite{international2011declaration}. However, principles alone are not enough even in relatively well-understood industries such as bioethics and safety engineering let alone fast-evolving AI research. Often generality of these principles limits their ability to provide practical action plans  \cite{whittlestone2019role}. Nevertheless, there is value in standardization to some extent, these frameworks can act as a decent first step and provide a common language to follow more context-dependent study but there are not sufficient on their own. 








% On the other hand, democratic fairness aims to tackle a few problems that low-resource entities may face simultaneously. The envisioned goal in democratic fairness has three main components:
% \begin{enumerate}[noitemsep,topsep=0pt]
%     \item Compatibility with different fairness concepts.
%     \item Evolvability through different data distributions.
%     \item The efficacy of computation while reusing the pretrained initiator model.
% \end{enumerate}

% In fact, we aim to achieve an inclusive, and accessible deployment by mindful designing of initiator models and leveraging local knowledge. Democratic fairness empowers communities themselves to have more control over their lives. Therefore addresses the power imbalance of previously suggested proposals.







% Holistic view of, 
% While there has been initial progress, the studies were focus just on one aspect, 


% This has led to a fragmentation of research techniques, and it remains unknown how well advances on these individual branches connect to a broader view and how would it be executed.


%In the next section we will introduce the format of \textbf{Democratic Fairness} and why we believe it can respond to these problems.



% most of these are largely Eurocentric and do not really provide practical guidance on how AI researchers should incorporate the principles into their research agendas or practice


% create common language to do careful deliberation



% Impact assessment is necessarily a form of institutional governance, prone to rendering questions of ethics and justice as compliance exercises.


% the value of participation was limited:


% reciprocaal schemes and safety/privacy guarantees.


% utilizing participatory methods as a means of mitigating technical, ethical and sociotechnical risks

% Effective participation


% , the challenges of measuring the effectiveness of participatory efforts, and the challenges of balancing expertise (peer review) and incentives.

==> unused_files/03_Edge_cases_bis.tex <==
% \subsection{Democratic Fairness through Examples}
% To further demonstrate the need for these principles, below we present three illustrative set of examples of the complexity of adapting models cross-domains and why there is a need for the different guiding principles of democratic fairness to address them.

% \subsubsection{Affirmative actions: Not every protected group needs the same remedy!} \hfill \break
% Beyond the geo-cultural lens, even in a western account of morality, justice is not always about equality. Justice is relative to social structures. However, the current definitions of algorithmic group fairness such as equal opportunity and demographic parity are based on equalizing model performance metrics (e.g., accuracy, true positive rates) among different demographic groups \cite{zhang2022affirmative}. 
 
%  As political philosophers described, we are all carriers of particular social identities and we are encumbered at least to some extent, by the history, tradition, and culture of communities that we are part of \cite{macintyre2013after}. There is a large body of literature describing how affirmative actions benefit society as a whole \cite{sandel1998liberalism,rubenfeld1997affirmative}. Therefore, justice is a notion deeply rooted in historical context, social structures and identity. For example, affirmative-action policies vary from region to region and might take different forms, from targeted encouragement to hard quotas. Affirmative actions in the form of quotas in particular are fundamentally incompatible with other definitions in algorithmic fairness \cite{ho2020affirmative}. As an example, affirmative actions and reconciliation strategies towards indigenous communities in North America cannot be directly replicated in other places in the world, not only because of the historical context but also the demographic makeup of the populations \cite{schumann2019transfer}. 
 
%  %As a result, transferring fairness in ML across-domains becomes an even more arduous task.     

% Both values and facts about geo-cultural population composition can find their way to regulatory bodies and reflect in legislation as well.  This includes considering what specific sociopolitical goals a given AI system enforces. For instance, considering their specific goals in Austria, a risk assessment algorithm created for use in the public employment system has been described as guided by a philosophy of neo-liberal austerity in the social sector, which has been replacing the concept of the European welfare state \cite{allhutter2020algorithmic, bringas2022fairness}.

% Another case requiring changes in the definition of what is fair and inclusive are various extreme events. Namely war and natural disasters create waves of social changes including immigration and refugee influx toward host countries or regions thus changing their composition and demographic distribution. As a response, host countries often try to design new policies and programs promoting the integration of new members in schools and employment \cite{brannstrom2018lived}. Therefore, it is important to build models able to adapt to such high-stake changes in terms of data distribution and values.

% Accordingly, the design of a democratically fair ML process requires honoring diversity by giving the communities the chance to practice the fairness notion aligning with their regulations and ideologies. This includes affirmative actions, which require different algorithmic formulations, as well as leveraging local expertise to tailor suitable solutions.


% \subsubsection{Different annotation infrastructure} \hfill \break
% Labeling properly is an expensive operation, thus often offloaded to crowdsourcing platforms as a means to reduce its cost. However, a lack of standardized annotation agreements and incentives schemes can translate into neglecting the geo-cultural context, leading to biased and inaccurate labeling. In fact, the work of annotators naturally is informed by their personal values, as well as their cultural and historical background.  Based on the annotator's knowledge and their lived experience, data would be likely labeled by association or proximity causing  (or $P_{source}(Y|X) \neq P_{target}(Y|X)$). As an example of annotation mismatch, a study showed that the labels of brides and grooms photos from different countries in the Open Images dataset show Eurocentric bias, as the bride-groom images from Ethiopia and Pakistan are not labeled as consistently as images from the United States and Australia \cite{shankar2017no}. Moreover, Sap et al. \cite{sap2019risk} showed how a lack of expert annotators on differences in dialect can lead to racial bias in automatic hate speech detection models, an AI for a good application, potentially amplifying harm against minority populations.

% % Moreover, annotation quality is influenced by the priorities of actors in power \cite{miceli2020between}. The lack of standardization and guidelines in the annotation process for instance {\todo might be because it is perceived as an optional?}

% Additionally, the crowdsourcing platforms often set low compensation for the annotators. Undermining data labeling work and "invisible workers" contribution \cite{irani2019justice} as opposed to considering it a collaboration also influences the annotation process and quality of data. 


% In conclusion, different variables in terms of resources and values affect the quality and reliability of datasets' annotation. Part of the solution could be designing a more inclusive, standardized, and reciprocal collaboration process by integrating local expertise and enabling cross-validation among annotators \cite{chmielewski2020mturk}. 


% \subsubsection{Different problem manifestation: Proxies, correlations, and causality} \hfill \break
% Usually, there is a metric assessed by the conductor of the research or common practices in the field that defines how to approach the problem at hand given the individual or collective constraints. In real-world, local domain statistical knowledge and expertise are key to formulating problems and corresponding data and ML pipelines. 
% For instance, which groups are considered as a minority varies depending on the context \cite{moreidentities, schumann2019transfer}. Local knowledge is then required to determine which demographic attributes to include in the dataset and which ones to focus on for the fairness evaluation. Such attributes might not always be available, thus additional knowledge is necessary to conceive proper solutions, such as choosing adequate proxies. Some examples include zip code as a proxy for race \cite{noauthor_using_2023}. While these proxies are adequate for some locations, they do not generalize well to other parts of the world. This relational mismatch of chosen attributes may cause a problem when casual reasoning of the problem is done with no local and domain expertise.
% Further, the assigned proxy can neglect the historic context, Obermeyer et al.\cite{obermeyer2019dissecting} showed that despite the belief that the health care cost appears to be an effective proxy for needed care by some measures of predictive accuracy, large racial biases arise from that assumption. Therefore, the historic unequal access to care among different subgroups in the US healthcare system is neglected.

% % or family structure as proxy for religion \cite{}

% Additionally, standardized frameworks are not fully compatible with various geo-cultural contexts, as certain phenomena manifest differently in different domains. As an example, in disease diagnosis and medical imaging, a challenging scenario is that under which the way anti causal prediction targets (e.g. disease status) physically manifest in the anatomy changes between domains. This cannot be corrected without strong parametric domain-specific assumptions on the nature of these differences \cite{castro2020causality}. 

% % Additionally, in a problem setting there might be differences between the relationship of attributes in the source and the target domains when transferring a model to a different geo-cultural context. 

% In general, an ML problem's formulation and hypothesis vary depending on the conductor's knowledge and values and might be subject to local regulations and protocols. The problem formulation then impacts all the ML processes starting with data collection, measuring and processing, feature selection, to model design. As the problem formulations highly depend on the context, local expertise is highly required to ensure an adequate model formulation, in addition to the alignment of the models with the different local regulations. 



% % This can be translated to the introduction of new attributes to the algorithmic system due to these high-stake events, not only ($A_{target}^i \notin A_{source}$), but all other attributes ($X_{target}^i \notin X_{source}$). Such variances can also require redefining the fairness in the algorithms based on raised situations.

 


% % \subsubsection{Emerging new protected groups}

% % Different extreme events, such as war and natural disasters create waves of social changes including immigration and refugee influx toward host countries or regions thus changing their composition and demographic distribution. As a response, host countries often try to design new policies and programs promoting the integration of new members. Therefore, it is important to build models able to adapt with such changes in terms of data distribution and regulations.

% % This can be translated to the introduction of new attributes to the algorithmic system due to these high-stake events, not only ($A_{target}^i \notin A_{source}$), but all other attributes ($X_{target}^i \notin X_{source}$). Such variances can also require redefining the fairness in the algorithms based on raised situations.
% % %{\todo add examples}

% % {\pointer Brännström et al.\cite{brannstrom2018lived} studied the rhetoric of policy reforms and its effects on the integration of new immigrants in Sweden. They raise attention to the dynamic nature of this integration and draw links between personal, organizational and policy domains from the standpoint of immigrants and government in various ways including labor market and employment opportunities. The authors reported many nuances and the ways in which these transforming policies are implemented locally. }

% % {\todo add conclusion about DF principles}


% %There is usually a metric assessed by the conductor of the research or common practices in the field that defines how to approach the problem in hand given the individual or collective constraints. 
% % Usually during data collection and processing, there is a wide range or poll of the representation states or easy-access proxies used for measuring an attribute. {\pointer These variations give rise to inconsistency and shifts across different datasets.} On the other hand, 

% % \subsubsection{Attributes correlate together differently in different domains}

% % Lets assume in a problem setting there are differences between the relationship of attributes in the source and the target when transferring a model to a different geo-cultural context. An example would be that in the most common studies, zip code is a proxy for race, or family structure is a proxy for religion whereas this could be true for some locations and does not generalize well to other parts of the world. This relational mismatch of chosen attributes may cause a problem when casual reasoning of the problem is done in an entirely non-expert, imposing their own bias.

% % {\pointer This is a well-studied example is in medical imaging that may result from the use of different scanners, devices or imaging protocols and standards across different countries and even medical sub fields. These factors would result in variances in data and its quality that do not necessarily give us added perspective on the subject \cite{castro2020causality}.

% % \afaf{How does this example fit in this context?}
% % For instance, high obesity is generally predictive of heart disease, but this relationship may not hold for smokers who have lower rates of obesity and higher rates of heart disease \cite{wiles2021fine}.

% % In another example, \cite{obermeyer2019dissecting} showed that despite the belief that health care cost appears to be an effective proxy for care need by some measures of predictive accuracy, large racial biases arise from that assumption. This assigned proxy neglects the historic unequal access to care among different subgroups in the US healthcare system.}



==> unused_files/04_Democratic_fairness_bis.tex <==
% The interconnection of decision consequences of different elements such as the data characteristics, the model's architecture and design, and the deployment structure on each other urges us to take a more holistic approach. 




%Picturing data composition, model design and deployment structure simultaneously provide us with better positioning and understanding of the relationship between technical and non-technical aspects of an understudied sociotechnical systems.

% A range of questions can be answered in this setting including "how the generalization characteristic or specification capabilities of a model should look like" or "what would be the true cost of running a reliable system" and "what would be an ideal labor market composition for a specific adaptation".

% To better assess effective design, deployment strategies and harm mitigation interventions, the various heterogeneity axes should be handled simultaneously. This requires a system-level view of the ML pipeline, alongside granular-level knowledge of the particularities of the context where it will be used.  More specifically, this holistic, yet specialized view, can give foundation for a customized design of the ML pipeline and accurate estimation of its costs. 

% In this section, we define and present the democratic fairness framework that can host a holistic approach to fair ML while taking into account the heterogeneity and scarcity challenges. Our view would highlight the importance of equitable participation of different types of stakeholders in the process to be able to design a sustainable model. We first define main principles that such a framework should inhere. Next, we introduce its format and assumptions.



% Democratic fairness is a framework aiming to bridge the gap between data, resources and values in the ML pipeline. We desire such a framework to bring a holistic, inclusive, accessible, and sustainable design. As a short description, democratic fairness aims to provide a two-level framework consisting of initiator models alongside rigorous documentation, so that communities can use that model and adapt it to their local capacities and preferences.


% % This can be achieved by leveraging local knowledge and empowerment. 
% % Accordingly, 

% We define the following guiding principles for the democratic fairness framework as follows:   

% % As a short description, the ultimate goal of democratic fairness is to provide an initiator model directory alongside rigorous documentation, so that communities can use a model from the directory and adapt it to their fairness conception and data composition given their possibly limited resource. 

% %\afaf{Please feel free to add details to these principles or to make suggestions :) }
% \begin{itemize}[leftmargin=*]
    
%     \item \textbf{Honoring diversity and inclusion of different perspectives:}  Communities should have the choice to adopt a model aligning with their fairness perception, values and regulations. 
%     The respect that results from deliberating and being exposed to different moral compasses and including them is more adequate for a pluralist society \cite{sandel1998liberalism}. It also builds a deeper level of trust in the final model's decisions.
    
%     % This not only adapts the process to the different regulations and values, but it also promotes respect among the different stakeholders and insures trust in the final model's decisions.  
   
%     \item \textbf{Local empowerment:}
%     Local empowerment stems from the degree of impact that local stakeholders have on a project \cite{birhane2022power}.  
%     An external AI team lacks the lived experiences required to comprehensively approximate and account for the needs of various stakeholders, especially already marginalized communities. As a result, it is necessary to include the local knowledge created by the people directly affected by the ML models in data collection, processing, model design and adaptation. The democratic fairness framework invites us to empower communities themselves to have more control over their lives. 
  
% %    \item \textbf{Inclusion:}  {\todo add details}
% %    Generally a broad range of participants plays an important role in ML pipeline but the reward of this participation is disproportionately distributed among different stakeholders. 
 
    
%     \item \textbf{Accessibility and portability:} Models should be efficiently reusable by different communities and compatible with different infrastructures. The status quo of AI is that it is a highly specialized field, where only select few practitioners have the expertise to design and maintain models. Furthermore, additional barriers are created by hardware  disparities. 
%     Two key principles to ensure accessibility would be to adequately document the data and models to insure reliable reusability by different communities. Additionally, designing adaptable models and deployment strategies \cite{8763885} should be of high priority in democratizing AI as whole and algorithmic fairness in particular.
%     Further, portability is particularly necessary to adapt to resource heterogeneity. For instance, a model or set of models intended to be reused elsewhere should be compatible with different tech stacks \cite{ahmed2020framework}. 
    
%     \item \textbf{Sustainability:} Democratic fairness aims to encapsulate sustainability and adaptability. Indeed, given the dynamic aspect of society, data and the emergence of new environments and regulations, it is necessary to design models that are easy to retrain and evolve through different changes. Designing workflows that allow updates with clear documentation plays an important role. 

%     % \item \textbf{Holistic view:} Different aspects regarding data, values, and resources are intertwined and cannot be easily disentangled. The way they interact is complex and requires a holistic view throughout the ML model's lifecycle. The different principles of democratic fairness should also be maintained in the different stages of the ML project.  
% \end{itemize}


% \input{03_Edge_cases_bis} 


% \begin{itemize}[leftmargin=*]
%     \item \textbf{Large Language Models} \hfill \break

% \end{itemize}

% Here for simplicity we start with first layer of exploring these axes in LLMs as they are presented by most of tech companies.  




% \subsection{A Framework for Democratic Fairness}
% \maryam{The points below are just placeholders and are not finalized yet}

% We picture two types of sharing/exchange conditions among different entities, which are:
% \begin{itemize}
%     \item Direct collaboration
%     \item Indirect collaboration via trusted party 
% \end{itemize}

% Further we define five types of sharing/exchange context among different entities, which are:
% \begin{enumerate}
%     \item Model-model sharing, each side shares some intel about their models (algorithm, latent space, etc.)
%     \item Model-data sharing, one side shares model-related intel and the other one shares partial or selected versions or agreed-upon portions of their processed data
%     \item Model-compute sharing, one side shares storage, cluster, etc. and the other some intel about their model
%     \item Data-data sharing, partial or agreed-upon data sharing
%     \item Data-compute sharing
% \end{enumerate}We picture two types of sharing/exchange conditions among different entities, which are:
% \begin{itemize}
%     \item Direct collaboration
%     \item Indirect collaboration via trusted party 
% \end{itemize}

% The role of the trusted party is: (it is somehow the same analogy of mimicking a potential government role like STAT Canada, etc.) We also quickly will mention incentives for each entity to cooperate with the trusted party (which is a choice). 

% \begin{itemize}
%     \item Providing local leadership
%     \item Concluding insights on trends and providing oversight (which can be done partly by automation and ML)
% \end{itemize}

% For the verifier, the role of the verifier is local and global audit and verification based on regulations and agreements among different entities.

% \end{itemize}

% Next, we discuss already existed techniques that can be used and laveraged .
% \subsubsection{Assumptions}
% Under the democratic algorithmic fairness principles, communities should have the choice to use ML for automating decision making in high stakes applications \cite{bygrave2020machine}, in addition to sovereignty on their data \cite{rainie2019indigenous}. Additionally, many data protection laws \cite{} and data sovereignty agreements back these rights \cite{}. Such laws were crafted to counter the abuse in power in ML and protect end users right to privacy. Accordingly, we assume that communities' data are private and cannot be accessed by the initial entity. {\todo say that there is an agreement, monetary or something }

% To define the framework, we assume that an initial entity is to transfer its model to a community or a small institution. 

% We make the following assumptions:
% \begin{itemize}
%     \item \textit{Communities' data are private and cannot be accessed by initial entity:}  \cite{rainie2019indigenous}

%     \item \textit{There is a publicly available library of crowdsourced  fairness notions.} 
%     {\todo add explanations}
%     %\rohan{Maybe this would be clear for someone who has read the entire paper, but, to me it wasn't very clear "who" has to have access to this fairness library}
%     \item \textit{Initial entity in source domain is resourceful.}     {\todo add brief explanation}
% \end{itemize}

% \golnoosh{Why these assumptions? can you explain them? (you can also get back to them in the limitation section)}
% Sure, I will get back to them in the limitation section, it seems better to include them there.

% \subsubsection{Format}
% The general idea is that the resourceful entity will build a library of models (called an initiator model directory) based on different fairness notions that later communities can directly use, fine-tune based on their preferences and resource capacity. Accordingly, we define two stages for model training: 1) Initiator models training and 2) Adaptation stage. The end goal of democratic fairness is collective learning of multiple tasks, in order to accelerate single task adaption later. Figure. \ref{fig:schematic} illustrates how data, resources, and values come into play in democratic fairness and how the process in envisioned in a simplified manner. 
% \begin{itemize}[leftmargin=*]
%     \item[1.] \textbf{\textit{Initiator models:} }
% The democratic fairness framework aims to honor the diversity of fairness notions as well as accessibility and portability. To achieve this, a tractable solution is to train a set of models on a library of fairness notions and make them available to communities desiring to use them. The various fairness notions can be crowdsourced by experts belonging to different communities based on regulations and values. 
% % By providing a library of pretrained models to communities, we aim for a faster yet reliable adaptation.
%  Moreover, to ensure that the models can be easily reused, model documentation \cite{mitchell2019model} should be provided. The documentation should also include which fairness notion was used and describe the used dataset. 
% % In fact, since data collection for different tasks is a slow process, using pretrained model provides a good starting point for communities pending building larger datasets. 
% The models should be designed and trained with domain change in mind. Accordingly, the models should be ready to use, or easy to adapt, as data collection and training might not be affordable. 
% A first step towards this is to provide a models directory that can be easily fine-tuned with few data samples. In fact, extensive experiments in \cite{wiles2021fine} showed that pre-training is a powerful tool across different shifts and often provides a strong boost in performance in downstream tasks. 
  
% %It is worth mentioning that, there is a growing effort on establishing iterative processes and curating community-centered public datasets, so that communities benefit from more incentive-neutral, responsible and accurate datasets \cite{sefala2021constructing}.
    
%     \item[2.] \textbf{\textit{Adaptation stage:} }
% While this is optional, the ability to adapt and fine-tune the models locally is necessary for model sustainability and accessibility.  Indeed, temporal shifts in the data, alongside possible changes in regulations and laws, would require retraining or completely changing the model. Local experts can implement drift detection mechanisms and trigger retraining whenever it is needed.

% Moreover, the embedded advantage of democratic algorithmic fairness, which is independent of the chosen ML methodology, is that communities are already in the loop, in the position of power, and are aware of their values, culture and data composition. So, there is already true prior knowledge at the adaptation stage on the targeted needs. Additionally, if the community has limited access to resources, the adaptation stage might include using compression techniques such as pruning \cite{blalock2020state} or knowledge distillation \cite{gou2021knowledge}.   
% It should be noted that documentation alone might not be sufficient to guarantee accessibility. As a result, providing support and training for ML practitioners \cite{deng2022exploring} is a necessary step towards democratic algorithmic fairness as a whole, and an efficient local model adaptation specifically.

% \end{itemize}


% \begin{figure}[t!]
%     \centering
%     \label{fig:df}
%     \includegraphics[width=0.5\textwidth]{images/democratic_fairness.drawio.pdf}
%     % \caption{Schematic of Democratic Fairness Framework. This figure illustrates the two stages required for obtaining a reliable model by communities and small enterprises. The initiator model directory would provide a series of models with a good performance on a defined library of fairness notions through which communities can adapt to their local preferences and resource capacity. In this process we want to maximize the support that initiator model}
%     % \label{fig:schematic}
% \end{figure}

% While the scale of implementation and context of the fair algorithm matter, overall, managing the balance of personalization and maintenance of social order at the larger scale is challenging and requires contributors from different disciplines \cite{mccann2004individualism, sandel2020tyranny}.


==> unused_files/05_Technical_enablers_bis.tex <==

 In this section, we discuss how several ML techniques and algorithms can enable democratic fairness, alongside some of their possible limitations.

\subsection{Initiator Model Directory}

The initiator model can be one or multiple models trained on a library of fairness notions. Multi-task learning, meta-learning, federated learning, and fair representation learning can be used to build the initiator model directory. Next, we will explain each approach in detail.

\golnoosh{Regarding the figure, we need to be careful about having a model directory that collects the data or having any sort of a centralized server/model/database/value system. }

\golnoosh{It would have been ideal to present a visual representation of these models and make it easier for the reader to compare them and grasp the advantage and disadvantage wrt the proposed framework. If adding a visual comparison is difficult, we need to present such comparison in a table format. This survey is a contribution, and it should have added values, but in the current format, this message that there are gaps but each approach has its own advantages is not delivered well. It reads more like related work rather than the promise of this work as technical enablers.}

\begin{itemize}[leftmargin=*]
    \item \textbf{Multi-task learning} is a problem in which multiple tasks are jointly learned by a shared model \cite{crawshaw2020multi}. While the task definition is dependent on the context and the targeted application, in the standard multi-task learning setup tasks are assumed to be defined on the same data distribution, but with different objectives \cite{caruana1997multitask}. A common architecture in multi-task learning consists of a shared component and multiple heads dedicated to each task \cite{zhang2014facial, dai2016instance, ma2018modeling, liu2019end}. Using multiple learning objectives or auxiliary tasks \cite{jaderberg2016reinforcement}, the goal is to have the shared component learn better representations that are useful for all downstream tasks, with the different tasks being different fairness notions. However, this approach is not readily applicable to problems with conflicting tasks.
    
    % Common approaches for alleviating this challenge include loss weighting \cite{gong2019comparison, liu2019loss}, gradient normalization \cite{chen2018gradnorm}, task scheduling \cite{bengio2009curriculum}, and gradient modification \cite{yu2020gradient, mansilla2021domain}. Most of the multi-task learning techniques encourage either parameter sharing or parameter tying among tasks \cite{wang2020generalizing}.
    
    Multi-objective optimization methods have also been applied to multi-task learning problems for optimizing multiple conflicting learning objectives \cite{sener2018multi}. Since in multi-objective optimization problems there is not necessarily a solution that maintains a global minimum for all objectives, these methods aim to provide a computationally efficient approach for exploration of the Pareto front in the context of deep neural networks \cite{lin2019pareto, ma2020efficient}. Given that the objectives in democratic algorithmic fairness are not necessarily well-aligned, multi-objective learning algorithms can be a promising solution for finding the initial model parameters. 


    
    \item \textbf{Meta-learning} includes any type of learning based on prior experience with tasks other than the target task \cite{hospedales2021meta, naik1992meta, thrun2012learning}, where a task is defined as a tuple of data distribution and loss function. A task in the case of democratic algorithmic fairness might characterized, for instance, by a loss function which includes a regularizer based on the corresponding fairness notion. 
    The main assumption is that tasks are drawn from a fixed distribution. At meta-training time, $N$ tasks are drawn from the task distribution, and the meta-learning algorithm attempts to find a model such that, when faced with a new task, that model can quickly adapt.
    One of the well-known types of meta-learning is Model-agnostic meta-learning (MAML). MAML learns a model parameter initialization that generalizes better to similar tasks \cite{finn2017model}. Learning search steps by a meta-learner can directly guide the learning algorithm. If we consider fairness notions as the different tasks to tackle, then the challenge would be to align the incompatible notions on top of adapting to different distributions. This might be a challenging task as training with different loss functions has been understudied compared to different data distributions.

    \item \textbf{Federated learning (FL)} consists of multiple distributed collaborators that try to solve a common problem under the coordination of a central aggregator while keeping data private \cite{zhang2021survey, kairouz2021advances}. Usually, the central model is built on the simple aggregation of collaborators learning parameters which do not necessarily guarantee the best performance for all collaborators. FL can allow entities with similar fairness definition to train a shared model \cite{chu2021fedfair} that can be later fine-tuned using several personalization techniques \cite{tan2022towards}. It can also be leveraged by communities in the adaptation stage to benefit from collaboration while keeping their data private.
    Additionally, it can be used in concurrence with the other techniques, such as multi-task learning \cite{smith2017federated,marfoq2021federated}, meta-learning \cite{fallah2020personalized}, and rank learning \cite{mozaffari2021frl}, to enable training on different tasks in a privacy-preserving manner. Indeed,  FL was initially designed to avoid sharing the local data. This privacy-preserving aspect of FL can be further enhanced using other techniques such as differential privacy\cite{wei2020federated}  and secure multi-party computation for aggregation \cite{bonawitz2016practical}. 
    % \rohan{Is the discussion of privacy a conscious choice here? It seems to be slightly deviating from the Fairness aspects mentioned before. Or maybe rephrasing it to show that FL has benefits of Meta learning/multi task learning along with privacy could help in the reader to understand why it is helpful}

    % Although, the definition of a task in meta-learning would include variation in loss functions but prior work focus mainly on different distribution variations. {\todo add comments about data + resources}
    % \item \textbf{Hypernetworks} refer to neural networks that generate another neural network, referred to as the main network, based on some input parameters \cite{ha2016hypernetworks}. The input is often selected as a pre-determined context or task parameters \cite{von2019continual} for conditional generation of the main network. Recent works show that hypernetworks are a suitable choice for meta-learning \cite{zhmoginov2022hypertransformer, beck2022hypernetworks} and transfer learning \cite{rezaei2022hypernetworks, sendera2023hypershot}. In the context of democratic fairness, a hypernetwork can be regarded as an initiator model that is trained to generate main networks fine-tuned with the different fairness notions for later adaptation by communities. \rohan{Do we expect communities to use the fair trained hypernetworks to re-initialize the networks for the communities? It might be helpful to point out how this adaptation is different from the ones discussed above. That is the need to have a fair hypernet which will possibly give a better init to the new adaptation model for the community} 
    

    \item \textbf{Fair representation learning} \cite{pmlr-v97-creager19a} allows for the adaptation of the same representation to different classification tasks with new target labels and subgroup definitions. The key idea is to use a compact encoding of the dataset using a variational auto-encoder for instance. The representation can be modified at test time, which can help bypassing the need to redefine the problem locally for new protected groups. These representations can also enhance the privacy but at the cost of mistrust from users and regulators \cite{mcnamara2019costs}, as an inferior fairness-accuracy tradeoff and higher individual unfairness are incurred.  



\end{itemize}

{\todo Add the final table}

\golnoosh{what about post-processing, personalization or fine-tuning methods?}
\subsection{Adaptation stage and specialization capability}

At the adaptation stage, while accessing the initiator model alongside documentation of data and model design, communities can assess the adaptation techniques needed to adjust the initiator model for their application. Since we assume their selected fairness notion is already in the poll of accounted tasks in the initiator model design, this stage will target minimizing resource costs while dealing with small datasets. The techniques needed for this stage can be found in literature including transfer learning, few-shot learning and knowledge distillation.

\begin{itemize}[leftmargin=*]

    \item \textbf{Transfer learning} \cite{zhuang2020comprehensive} is used to leverage knowledge from a source domain, to improve and accelerate the learning performance in a target domain. The goal is to obtain transferrable features that can be used for various downstream tasks. It can be particularly useful for small communities with limited training samples, however, the transferred knowledge does not always bring a positive impact on new tasks. If there is little in common or a goal mismatch between domains, knowledge transfer could be unsuccessful or even hinder the learning on the target task. 
        
    \item \textbf{Few-shot learning} studies the performance of a model to make predictions downstream on a small dataset or few examples, as few as one example per class \cite{fei2006one}. Few-shot learning methods often follow three directions to obtain their goal: the prior knowledge can be constructed by augmenting data, constraining the hypothesis space of the model, or altering the search strategy in the hypothesis space \cite{wang2020generalizing}. In the democratic fairness framework, we can for instance use multi-task learning and few-shot learning in tandem where we place the few-shot tasks as target tasks, since communities would have data scarcity, and the rest as source tasks. Notably, meta-learning algorithms \cite{finn2017model} are also a promising choice for achieving few-shot learning, as the meta-learning problem formulation naturally encompasses that of the few-shot learning.
    
    \item \textbf{Knowledge distillation} aims to effectively learn a small student model from a large teacher model \cite{gou2021knowledge}, thus allowing both the transfer of knowledge and adapting to limited resources. This is achieved by extracting potent knowledge from the teacher and using it to guide the training of the student.  By considering small or new communities' tasks as student tasks in knowledge distillation, we can adopt it for the democratic fairness framework. It has been recently shown that using knowledge distillation through the usage of soft-labels can help achieve a better fairness-accuracy trade-off for several tasks and fairness notions \cite{chaifairness}. Nonetheless, a deep understanding of generalization and capacity of knowledge distillation, especially how to measure the quality of knowledge or the quality of the teacher–student architecture, is still limited \cite{gou2021knowledge}. Furthermore, the effect of knowledge distillation on fairness notions is still limited. 

    \item \textbf{Continual learning} refers to the ability of a learning agent to continually learn and adapt to new scenarios over the duration of their lifetime, ideally without forgetting the tasks that were learned initially \cite{khetarpal2022towards}. As a result, continual learning algorithms are an appealing choice for handling several types of distributions shifts that occur in the democratic fairness framework, as discussed in Section \ref{sec:data_het}.

    \item \textbf{Fairness post-processing approaches}

\end{itemize}


% \subsubsection{Discussion \& Limitations} \hfill \break
% A first step towards bridging the dissimilarity gap is to build a models directory supporting a library of fairness notion. The model directory can be composed of different models corresponding to each definition, or a single powerful model using meta-learning or multi-task learning.

% However, the typical scenarios for meta-learning and multi-task learning are restricted to correlated tasks, and they focus on maintaining a certain level of generalization and performance for each learning task. In the case of fairness notions, even with commonly used statistical notions, in addition to the existing trade-off between accuracy and fairness, several notions of group fairness conflict with one another \cite{kleinberg2016inherent, chouldechova2017fair}. Therefore, to be able to design a foundation that can hold premises of democratic fairness for such conflicting tasks, we bring attention to conceptualizing task similarity or task distance. We intend to identify similar tasks and group them together in the learning process of the initiator model, so that one can make sure that each team of tasks can converge to a meaningful point.

% There exists several methods that can be used to build a democratic algorithmic fairness framework. However, transferring knowledge and fairness across domains depends on the tasks' similarity.

% Relatedly, the initiator model directory can be constructed as a form of a hypernetwork \cite{ha2016hypernetworks} that generates community-specific networks that perform well for few-shot or zero-shot transfer \cite{zhmoginov2022hypertransformer, sendera2023hypershot, rezaei2022hypernetworks}. The initiator model directory can also be built in a decentralized way using federated learning for instance. Another possible approach is to provide a model that learns fair representations which can be adapted to different demographic compositions. Yet, fairness notions are evolving and new definitions of algorithmic fairness emerge frequently \cite{verma2018fairness,wong2020democratizing}. Accordingly, continuous support for the initiator models directory is necessary. Additionally, a study for the possibility of transferring knowledge even under different fairness definitions can be a promising direction. Yet, establishing a compatibility assessment of different definitions might be challenging. Moreover, evaluating the quality and usability of the initiator model would be left to the target communities. 

% \afaf{I will look for references and see if it can fit elsewhere (like the initial definition maybe), I feel like we need to make it look possible in the beginning, and here discuss that a way to ensure it is still not established irl. And it is okay to repeat it in the conclusion as one of the takeaways}

% Additionally, adopting the models locally requires adapting to the resources and data scarcity. As a result, transfer learning and few-shot learning can be used to quickly train the models locally. Furthermore, knowledge distillation for example can allow the target communities to design smaller models that fit their resources. Nonetheless, an end-to-end study of how the fairness-accuracy trade-off is affected by the domain change and resource adaptation is still lacking.
% % \rohan{The discussion and limitation are entangled in this paragraph and it is tough for the reader to understand which is a limitation and which is not.} 
% This challenge will remain in democratic fairness throughout different levels. Firstly, at initiator model stage, we face conflicting tasks since even with commonly used statistical fairness notions we are aware that on top of the existing trade-off between accuracy and fairness, several notions of group fairness conflict with one another \cite{kleinberg2016inherent, chouldechova2017fair}. Other level that we face this challenge is when communities want to adapt to their dataset. Having a pre-defined library of fairness notions at the beginning and prior knowledge that communities have about their data composition would help tremendously.

% By identifying similar tasks and group them together in the learning process of the initiator model, so that we can to some extent make sure that each team of tasks can converge to a meaningful point for them. Then we treat every member of the team under the concluded united identity. Further, we can assign weights to the final teams, so that we can have more control over determining each team's impact, which will get reflected in the pareto fronts.

\subsection{Limitations of democratic algorithmic fairness}

{\todo assumptions}

{\todo feasibility and cost -- maintenance cost}

Aside from the technical part of the democratic fairness framework, from a macroeconomics perspective, we recognize the lack of incentives or readily business models for resourceful entities to get interested and develop the initiator models. Generally, we believe there are many moving pieces in the AI governance ecosystem including regulation that should advance together to be able to observe meaningful progress in either of them. Regulation can curb the dominance of resourceful entities and pave new sustainable approaches for them to benefit from their resources while safeguarding the public interest.









% Weighted resampling works only with the source data, it either try to correct the marginal distribution difference by imposing a ratio, or to adjust the conditional distribution difference, or to do both \cite{weiss2016survey}. Feature-based approaches transform each original feature into a new feature representation for knowledge transfer. The objectives of constructing a new feature representation include again minimizing the marginal and the conditional distribution difference, preserving the properties or the potential structures of the data, and finding the correspondence between features.

% A common approach to transfer learning under distribution shift is to fine-tune the last few layers of a pretrained model, preserving learned features while also adapting to the new task.
 






==> unused_files/05_technical.tex <==
%In this section, we discuss the current landscape of common scenarios and their respective techniques in the field while describing their gaps with regard to simultaneously treating the three axes of heterogeneity (data, values and resources), as well as the feasibility of control that each scenario gives to different stakeholders. 


Different stakeholders especially end-users, communities, and small entities have little to no control on how to design, participate, intervene, or adapt the models to their needs, environment, and resources. One of the assumptions that we make in order to explore these scenarios is that values are considered tangible means for ML pipeline design. 

%Afaf:
%The problem formulation 
%Data collection
%Participatory design
%Choice of fairness definition

For instance, algorithmic fairness notions are usually used in processing techniques as a constraint on an optimization problem, as the regularizer in the loss function, or as an objective itself in a multi-objective setting \cite{zafar2017fairness, choi2020learning, martinez2020minimax, agarwal2018reductions}. 

% partnership

In this section, we discuss the current landscape of ML pipelines and the techniques used to handle the three axes of heterogeneity (data, values and resources). The discussion also includes the level of control that each technique gives to different stakeholders. 
%Although we acknowledge this is a naive take on values and doesn't consider different values that different communities hold regarding the methodology of research, collaboration agenda, evaluating, etc.

%Summary of what's coming next

\subsection{Data sharing}
A way of being included and represented in the training dataset is data-sharing. 
Data can be shared in different ways
but raises privacy and sovereignty concerns...






\subsection{Large Pretrained Models}

{\afaf since this is what we criticize in the beginning of the paper, this part should focus on fine-tuning and multi-task learning. The narrative would be that in a scenario where resourceful entities are willing to share the model (be it a foundation model or a multi-task model etc). I think in this case we can also add domain adaption to this part. }
% The first category of model development, which is currently the dominant trend, describes the scenario in which resourceful companies \emph{choose} scaling as their strategy.

Currently, resourceful companies choose scaling as their strategy.
For instance, large language models ????

%Large language models are the famous example. Some more studied areas of LLM include but are not limited to machine translation, conference resolution, hate speech and toxicity detection, fact-checking, Information extraction, Information classification and summarization, as well as interactive experiences. Each of these categories redefines itself and the risks that it may carry when applied to different domains and implementation scales. There is overarching ambiguity and tendency around studying LLMs separate from their context and actual application which makes us more excited about their advances rather than picturing their risks before causing harm especially when there is unassigned accountability about them. This brings the need for specification and understanding of how the three axes of heterogeneity, data, value and resources play a role more strongly in each context.


\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{images/control.drawio.pdf}
    \caption{Control ?}
    \label{fig:control}
\end{figure*}




While large pretrained models have demonstrated multi-task \cite{radford2019language} and few-shot \cite{brown2020language} learning abilities, their training and development requires a high amount of compute and storage capacity \cite{bommasani2021opportunities}.

%{\afaf is this really a result?}
%As a result, these enterprises end-up embedding their values in the process of building their proprietary tools.

Considering the fast-paced and competitive culture of AI research, lack of regulations and accountability, lack of public literacy, investment of these companies in public relations, insisting on AI capabilities and exhibiting futuristic views, the narrative of developing large pre-trained models is already distorted. The issue is exacerbated particularly due to the level of power and influence that these companies have. In this scenario, at best, we can hope that such powerful entities would include different values and data compositions during the training phase, through techniques such as multi-task learning.


First, we discuss this scenario from the feasibility and reliability perspective with respect to generalizability and embedded values. \emph{Multi-task learning} is a problem in which multiple tasks are jointly learned by a shared model \cite{crawshaw2020multi}. While the task definition is dependent on the context, in the standard multi-task learning setup tasks are assumed to be defined on the same data distribution, but with different objectives \cite{caruana1997multitask}. A common architecture consists of a shared component and multiple heads dedicated to each task \cite{dai2016instance, liu2019end}; using multiple learning objectives or auxiliary tasks \cite{jaderberg2016reinforcement, liebel2018auxiliary}, the goal is to have the shared component learn better representations that are useful for all downstream tasks.

However, large pretrained models have shifted this paradigm as they can achieve reasonable performance on numerous tasks by training a single large model on a diverse enough dataset \cite{radford2019language}. 

Regardless, we can consider adding different values (e.g., fairness notions) as different tasks in a multi-task learning setup. However, this approach is not readily applicable to problems with conflicting tasks such as fairness notions. The impossibility theorem in fairness \cite{saravanakumar2020impossibility} states that the common statistical group fairness notions cannot be satisfied simultaneously. 

Multi-objective learning methods are one possible solution to conflicting learning objectives \cite{sener2018multi} by providing computationally efficient approaches for exploration of the Pareto front \cite{lin2019pareto, ma2020efficient}. As a possible use case, fairness notions can be considered as different objectives in a multi-objective learning problem \cite{martinez2020minimax, padh2021addressing}. In this case, the challenge would be to align the incompatible notions on top of accommodating to different data distributions and guaranteeing the convergence of the model to some meaningful point(s) under this condition. 

Furthermore, even aside from the mentioned challenges regarding feasibility, in many cases, even resourceful companies do not have long-tail or unique datasets that encompass smaller communities as well as a library of all fairness definitions that communities consider. This will require different communities to give up their data autonomy and agency in order to be included in the development process of the large model. This hidden contract, which on the surface may appear volunteer-based and reciprocal to some extent, has many similarities with colonial era agreements where the benefits were heavily skewed in favor of the powerful. It also questions the legitimacy of the initial consent as there are few choices for communities to be considered in this form of digital citizenship.  







% TODO: No oversight

% TODO: prompt engineering

% methods that measure or combat extrinsic outcome disparities may not align with stakeholder goals[Sahaetal.2020],and there is some evidence to suggest certainty pesof technicalinterventionmaybesimultaneouslyunsatisfiable [Corbett-DaviesandGoel2018;Kleinbergetal.2017],impossible[Lechneretal.2021],or mayeven exacerbate inequity[Xuetal.2021].

% transparency,especiallygiventhattechnicalmitigation methodsmaynotbeabletoachievetheintendedgoals.Morebroadly,claimsofbiasandbias mitigationmustbemadecarefullytoclearlycommunicatethestatusquotovariousstakeholders withdifferingexpertise(e.g.,applicationdevelopersbuildingontopoffoundationmodelsand policymakersregulatingthetechnology;[Nissimetal.2020]).

\subsection{Fine-tuning and Adaptation}
Communities can potentially finetune large pretrained models to better align them with their unique data and values. 

However, this is not often feasible as the weights of the model, training code, and any documentation on the original data or model design choices are not available, thereby limiting communities' ability in making necessary adaptations and resulting in a lack of control.

Generally, the development of these systems takes place in the context of late-stage capitalism, which romanticizes efficiency, scale and automation. The ethos of accumulation deviates attention from harms and underlying power concentration to the point that placing a democratic government in this scheme will be challenging.

If we assume that large pretrained models are open-sourced and well-documented, communities are able to further finetune them to fit their needs and values, using techniques such as transfer learning or knowledge distillation. 

\emph{Transfer learning} \cite{zhuang2020comprehensive, pan2010survey} aims to leverage knowledge from a source domain to improve and accelerate learning on a target domain. The goal is to obtain transferrable features that can be used for various downstream tasks, thus it can be particularly useful for small communities with limited data and computation. However, the transferred knowledge does not always bring a positive impact on new tasks. If there is little in common or a goal mismatch between the domains, knowledge transfer could be unsuccessful or even hinder learning on the target task, resulting in negative transfer, that is the performance and efficiency are actually worse than training from scratch on the target domain \cite{wang2019characterizing}.

\emph{Few-shot learning}, a specific transfer learning scenario, studies the performance of a model to make predictions downstream on a small dataset or few examples, as few as one example per class \cite{fei2006one}. Few-shot learning methods often follow three directions to obtain their goal: the prior knowledge can be constructed by augmenting data, constraining the hypothesis space of the model, or altering the search strategy in the hypothesis space \cite{wang2020generalizing}. While there are data and embedded value heterogeneity, we can for instance use multi-task learning and few-shot learning in tandem where we place the few-shot tasks as target tasks, since communities would have data scarcity, and the rest as source tasks. Notably, meta-learning algorithms \cite{bengio1990learning, schmidhuber1987evolutionary, finn2017model} are also a promising choice for achieving few-shot learning, as the meta-learning problem formulation naturally encompasses that of the few-shot learning.

From the feasibility perspective even if the pretrained model is elaborate, there are limits to what finetuning can do. Importantly, the effect of finetuning in the specfic case of large pretrained models is not yet fully studied and it is unclear to what extent a large pretrained model can be adapted to novel downstream tasks \cite{tran2022plex}. We can define finetuning capacity as the ability of a pretrained model to efficiently adapt to new tasks; the question then becomes how to increase the finetuning capacity and how to determine whether finetuning of a large pretrained model is cost-efficient and effective or generally how we define cost. While recent works \cite{ding2023parameter, tran2022plex} have tackled this important adaptation problem, the aforementioned questions call for further research to develop better evaluation benchmarks that can clear the ambiguity of the adaptation criteria, ease of computation, and efficiency of the adaptation process. 

% Questionable benchmarking
% Evaluation questions

    
Knowledge distillation aims to effectively learn a small student model from a large teacher model \cite{gou2021knowledge}, thus allowing both the transfer of knowledge and adapting to limited resources. This is achieved by extracting potent knowledge from the teacher and using it to guide the training of the student. Facing data and embedded value heterogeneity, one can consider small or new communities' tasks as student tasks in knowledge distillation. It has been recently shown that using knowledge distillation through the usage of soft-labels can help achieve a better fairness-accuracy trade-off for several tasks and fairness notions \cite{chai2022fairness}. Nonetheless, a deep understanding of generalization and capacity of knowledge distillation, especially how to measure the quality of knowledge or the quality of the teacher–student architecture, particularly on fairness notions, is still limited \cite{gou2021knowledge}. 




Regardless of the feasibility and evaluation question, more importantly, any post processing tweaks are in favor of reinforcing the need for a resourceful entity to build the initiator model in the first place without others having any control of its process, it reinforces the already existing power structure and our dependence on them. This will further exacerbate and widen the financial and technological divide between a few entities and the rest of society.

% stacking faulty ML
% The risks of stacking AI are twofold. First, if two algorithms that produce incompatible outcomes are integrated under the same system, they may not achieve optimal performance. Second, if many algorithms are combined, existing risks can be amplified or propagated. Privacy, fairness, explainability and other issues in a single algorithm could compromise the entire network (Dwork and Ilvento, 2018).

\subsection{Collaborative Training}
Another tractable solution is to opt for collaborative training, in which different entities (e.g., institutions, communities) can collaborate with each other through techniques such as federated learning, peer-to-peer and split learning.  

%it gives more control over data and more say in how to participate, how much to share... but if there is a values misalignment... hmmm

%The third category describes collaborative learning paradigms, in which different communities, institutions and entities can collaborate with each other through techniques such as federated learning, peer-to-peer and split learning. 

%Such techniques give more control to the different entities...

% Healthcare crisis collaboration as an example \hfill \break

% Bringing a scenario in which different hospitals around the globe want to conduct a research on Covid-19. 


% Data heterogeneity would include 
% \begin{itemize}
%     \item different instruments and measurement protocols 
%     \item different reporting/documenting criteria 
%     \item different demographics in terms of race and age
%     \item different collected proxies based on availability and 
%     \item different quantity and quality of data
    
% \end{itemize}

% Value heterogeneity would include 
% \begin{itemize}
%     \item different data privacy and consent protocols 
%     \item different provincial and state-wide discriminatory regulation
%     \item different methodology used 
    
% \end{itemize}


% Resource heterogeneity would include 
% \begin{itemize}
%     \item experties and consultation design budget
%     \item compute capacity
%     \item data size capacity 
    
% \end{itemize}



% free labor as the feedback loops. Whose ethics? Who decides and then who agrees to comply? 

% dana boyd.
% “We misunderstand ethics when we think of it as a binary, when we think that things can be ethical or unethical. A true commitment to ethics is a commitment to understanding societal values and power dynamics – and then working toward justice.

\emph{Federated Learning} (FL) consists of multiple distributed collaborators that try to solve a common problem under the coordination of a central aggregator while keeping data local \cite{mcmahan2017communication, zhang2021survey, kairouz2021advances}. This gives collaborators more control over their data, and allow very low-resourced collaborators to participate. The main assumption is that collaborators agree on model architecture, and then the central model is built on the simple aggregation of collaborators learning parameters. Therefore, the final product does not necessarily guarantee the best performance for all collaborators especially in light of their data and embedded value heterogeneity. 

FL can allow entities with similar fairness definition to train a shared model \cite{chu2021fedfair}. Additionally, it can be used in concurrence with other techniques, such as multi-task learning \cite{smith2017federated,marfoq2021federated}, meta-learning \cite{fallah2020personalized}, and rank learning \cite{mozaffari2021frl}, to enable collaborative training on different tasks. Moreover, while the premise of FL is to avoid sharing the local data, communicating the model updates throughout the training process with the aggregator can reveal sensitive information, but these privacy-preserving aspect of FL can be further enhanced using other techniques such as differential privacy \cite{wei2020federated} and secure multi-party computation for aggregation \cite{bonawitz2016practical}. 

Understanding and balancing the aforementioned concepts and their respective tradeoffs, both theoretically and empirically, is challenging. Using FL, one has control over its data and model parameters sharing (collaborators can choose if they like to partially participate through sketched or structured updates \cite{}), but it is not yet guaranteed that FL frameworks can accommodate different data distributions and orthogonal fairness definitions while maintaining efficient communication.

Trust building in the context of collaborative paradigms has been recently studied. Trust determines users’ willingness to participate in the training process in the first place. Studies indicate ensuring fair treat among users are the main trust builder factor \cite{li2019fair, hu2022federated, mohri2019agnostic}. 


%For instance, Mohri et al. \cite{mohri2019agnostic} proposed linear weighting the collaborators' distributions to create a target distribution, which is then optimized for worst-case scenarios to ensure fair treat of each collaborator.

\emph{Peer-to-peer learning} \cite{vanhaesebrouck2017decentralized, savazzi2020federated}, which can be considered as a subcategory of federated learning, describes horizontal communication. Unlike federated learning, there is no central aggregator, thus each collaborator relies on their compute capacity. Peer-to-peer learning allows direct communication among collaborators. This brings up the availability of compute capacity for each collaborator as well as the richness of their communication infrastructure as its importance is more pronounce in peer-to-peer schemes. 

\emph{Split learning} \cite{vepakomma2018split} is another collaborative paradigm in which a deep neural network is split into multiple sections, each of which is trained by a different collaborator. The network is trained by transferring the weights of the last layer, namely the cut layer, of each section to the next section while the data remains private and local. The gradients are back propagated at the server from its last layer until the cut layer. Only the gradients at the cut layer are sent back to each collaborator. The rest of back propagation will be completed locally. There are a few variations of split learning which allow keeping labels of different collaborators private as well. Generally, split learning enables collaboration under resource heterogeneity since it includes a facilitator server. On the other hand, from an ownership perspective, the server provider ultimately will keeps part of the network parameters required for inference which could be a concerning factor. From the data heterogeneity perspective, Li et al. \cite{li2023convergence} theoretically showed the convergence guarantees of split learning for non-convex objectives under data heterogeneity. 

To summarize, collaborative training approaches empower collaborators to control the privacy and sharing of their data and allows resource-limited collaborators to take part. There is still future work needed to analyze or operationalize their capabilities in data and embedded value heterogeneity. Certainly, a clear infrastructure or contract describing fair treatment, objective notions, communication infrastructure, etc. helps collaborators to make an informed decision on whether or not to participate.

% evaluation problem

% Each collaborator train for a few iterations with their local dataset until when a random collaborator sends out a request go get their latest model versions to generate new updates and the communication will be continued until reaching an opt to update its own model accordingly  


